Studying Taxonomy Enrichment on Diachronic WordNet Versions

Ontologies, taxonomies, and thesauri are used in many NLP tasks. However, most studies are focused on the creation of these lexical resources rather than the maintenance of the existing ones. Thus, we address the problem of taxonomy enrichment. We explore the possibilities of taxonomy extension in a resource-poor setting and present methods which are applicable to a large number of languages. We create novel English and Russian datasets for training and evaluating taxonomy enrichment models and describe a technique of creating such datasets for other languages.

==> tables.tex <==
\begin{table}[ht]
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{lrrrrrrrrrr}
    \toprule
\multicolumn{1}{c}{\textbf{method}} %& \textbf{dataset} 
& \multicolumn{1}{c}{\textbf{nouns}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}nouns \\ (restricted)\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}MWE \\ nouns\end{tabular}}}& \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}NE \\ nouns\end{tabular}}}& \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}short \\ words\end{tabular}}} & \multicolumn{1}{c}{\textbf{verbs}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}verbs\\ (restricted)\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}MWE \\ verbs\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}NE \\ verbs\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}short \\ words\end{tabular}}}
 \\\midrule
% \textit{baseline (fastText)}        & \multirow{3}{*}{\textit{WordNet1.6 - WordNet3.0}} &             0.2655                       & 0.2353                                          &   0.1978                                 & 0.2404                                          \\
% \textit{ranked (fastText)}          &                                   &       0.3347                             & 0.2853                                          &    0.2360                                & 0.2834                                          \\
% \textit{ranked + wiki (fastText)}   &                                   &    \textbf{0.3384}                                & \textbf{0.3179}                                          &        \textbf{0.2689}                            & \textbf{0.3192}                                          \\\midrule
% \textit{baseline (fastText)}        & \multirow{3}{*}{\textit{WordNet1.7 - WordNet3.0}} &                            0.3005        & 0.2141                                          &         0.1569                           & 0.1873                                          \\
% \textit{ranked (fastText)}          &                                 &      0.3522                                & 0.2666                                          &    0.1623                                & 0.1854                                          \\
% \textit{ranked + wiki (fastText)}   &                                   &          \textbf{0.3702}                         & \textbf{0.3036}                                          &  \textbf{0.2074}                                  & \textbf{0.2317}                                          \\\midrule
\textit{baseline (fastText)}         %\multirow{6}{*}{\textit{WordNet2.0 - WordNet3.0}} 
& 0.3253                             & 0.1485   &  0.3979  & 0.3275 &                       0.3193          & 0.1826                             & 0.1969   & 0.0423 & 0.2 & 0.3889                                        \\
\textit{ranked (fastText)}                                           & 0.3749                             & 0.2240  &  \textbf{0.4414} &  0.3869  &           0.3479                        & 0.1897                             & 0.2000     & 0.0257 & 0.2 & 0.2963                                     \\
\textit{ranked + wiki (fastText)}                                      & \textbf{0.4002}                             & \textbf{0.2578}         &  0.4068    &  \textbf{0.4501}    &       \textbf{0.3596}               & \textbf{0.2376}                             & \textbf{0.2366}    & 0.0362 & \textbf{0.4} &  \textbf{0.4112}                                    \\
\textit{baseline (BERT)}                                             & 0.2389                             &                        0.0996    &  0.2949     &  0.3296  &    0.2344       & 0.0973                             &                          0.1036           & 0.05 & 0.0 & 0.1389            \\
\textit{ranked (BERT)}                                              & 0.2383                             &                         0.1465      & 0.2364  &   0.3703  &   0.2271       & 0.1051                             &                          0.1167   & \textbf{0.0478} & 0.0 & 0.1334                    \\
\textit{ranked + wiki (BERT)}             & 0.2534                            &                     0.1828 &  0.2585    & 0.3415  &   0.2258   &                          0.1204                           &                       0.1394     & 0.0445 & 0.0 & 0.1112              \\                                        \bottomrule
\end{tabular}}
    \caption{MAP scores for the English datasets.}
    \label{tab:en_results}
\end{table}



\begin{table}[t]
    \centering
    \begin{tabular}{lrrrr}
    \toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{method}}} & \multicolumn{2}{c}{\textbf{nouns}}                                         & \multicolumn{2}{c}{\textbf{verbs}}                                         \\
\multicolumn{1}{c}{}                                 & \multicolumn{1}{c}{public} & \multicolumn{1}{c}{private} & \multicolumn{1}{c}{public} & \multicolumn{1}{c}{private} \\\midrule
\textit{baseline (fastText)}                         & 0.4348                              & 0.4210                               & 0.2759                              & 0.3335                               \\
\textit{ranked (fastText)}                           & 0.5129                              & 0.5071                               & 0.2734                              & 0.3357                               \\
\textit{ranked + wiki (fastText)}                    &                   \textbf{0.5329}                  &        \textbf{0.5404}                              &       \textbf{0.3490}                              &                  \textbf{0.3829}                    \\\midrule
\textit{baseline (BERT)}                             & 0.1443                              & 0.1377                               & 0.0724                              & 0.1186                               \\
\textit{ranked (BERT)}                               & 0.1942                              & 0.1846                               & 0.1094                              & 0.1271                               \\
\textit{ranked + wiki (BERT)}            &      0.2357                                    &         0.2179                              &          0.1432                          &                           0.1614           \\ \midrule\midrule
\textit{Yuriy (RUSSE'2020)}                          & \textbf{0.5590}                              & \textbf{0.5522}                               & 0.4032                              & 0.4355                               \\
\textit{cointegrated (RUSSE'2020)}                   & 0.4077                              & 0.4178                               & \textbf{0.4033}                              & \textbf{0.4483}               \\
\bottomrule
\end{tabular}
    \caption{MAP scores for the Russian datasets.}
    \label{tab:ru_results}
\end{table}


\begin{table}[ht]
    \centering
    \resizebox{\textwidth}{!}{
\begin{tabular}{lrrrrrrrrrr}
\toprule
\multicolumn{1}{c}{\textbf{dataset}} & \multicolumn{1}{c}{\textbf{nouns}} & \multicolumn{1}{l}{\textbf{nouns (restricted)}} & 
\multicolumn{1}{l}{\textbf{MWE nouns}} &
\multicolumn{1}{l}{\textbf{NE nouns}} &
\multicolumn{1}{l}{\textbf{short nouns}} &
\multicolumn{1}{c}{\textbf{verbs}} & \multicolumn{1}{l}{\textbf{verbs (restricted)}} &
\multicolumn{1}{l}{\textbf{MWE verbs}} &
\multicolumn{1}{l}{\textbf{NE verbs}} &
\multicolumn{1}{l}{\textbf{short verbs}}
\\
\midrule
\textit{WordNet1.6 - WordNet3.0}     & 17 043                    & 3 751     & 3 648 & 9 623  &        21                     & 755                       & 553 &               183 & 10 & 9                      \\
\textit{WordNet1.7 - WordNet3.0}     & 6 161                     & 1 840          & 1 682&        2 626   & 13             & 362                       & 224 & 120 & 10 & 8                                    \\
\textit{WordNet2.0 - WordNet3.0}     & 2 620                     & 890              & 582 & 1142 &    6                  & 193                       & 153 & 27 & 5 & 8\\
\textit{RuWordNet1.0 - RuWordNet2.0}     & -                     & 2 288           & -& -&    -                     & -                      & 525 & - & - & -\\
\bottomrule
\end{tabular}}
    \caption{Datasets statistics.}
    \label{tab:dataset}
\end{table}



\begin{table*}[ht]
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lrrrrrrrr}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{taxonomy}}} & \multicolumn{2}{c}{\textbf{synsets}}                  & \multicolumn{2}{c}{\textbf{lemmas}}                   & \multicolumn{4}{c}{\textbf{new words}}                      \\ %\cline{2-7} 
\multicolumn{1}{c}{}                                   & \multicolumn{1}{c}{nouns} & \multicolumn{1}{c}{verbs} & \multicolumn{1}{c}{nouns} & \multicolumn{1}{c}{verbs} &
\multicolumn{1}{c}{nouns} & \multicolumn{1}{c}{nouns (restricted)} & 
\multicolumn{1}{l}{verbs} & \multicolumn{1}{l}{verbs (restricted)} \\ \midrule
\textit{WordNet 1.6}                                   &             66 025              &              12 127             &             94 474              &       10 319                    &        -                   &     -             & - &-         \\
\textit{WordNet 1.7}                                   &             75 804              &              13 214             &             109 195              &       11 088                    &        11 551                   &     2 054 & 401 &323                      \\
\textit{WordNet 2.0}                                   &             79 689              &              13 508             &             114 648              &       11 306                    &        4 036 & 927 & 182                  &     60                  \\
\textit{WordNet 2.1}                                   &             81 426              &              13 650             &             117 097              &       11 488                    &       2 023 & 692 & 158                  &     116                       \\
\textit{WordNet 3.0}                                   &           82 115                &           13 767                &          117 798                 &        11 529                   &          678                 &  158 &   33 & 15                      \\ 
% \midrule
% \textit{RuWordNet1.0}                           & 29 297                    & 7 636                     & 76 817                    & 35 279 
% & - & - & -                    & -                       \\
% \textit{RuWordNet2.0}                           & -                    & -                     & -                    & - 
% & - & 2 288 & -                    & 525                       \\
\bottomrule
\end{tabular}}
\caption{Taxonomies statistics.}
\label{tab:statistics}
\end{table*}
